An Exploration of Possible Governance Models for the Future Global Gravitational-Wave Observatory Network

The construction of a global network of detectors is the cornerstone to scientific success for 3rd generation gravitational wave astronomy. If carried out with a vision to the future, the third generation implementation, in its infrastructure, technology base and governance can provide the point of departure for subsequent developments beyond the third generation, a path to the long and revolutionary future of gravitational wave astrophysics. The goal of this document is to lay out considerations that influence the optimal choice of governance and to lay out a possible path that can lead the community to an optimal governance model. This report is the six in a six part series of reports by the GWIC 3G Subcommittee: i) Expanding the Reach of Gravitational Wave Observatories to the Edge of the Universe, ii) The Next Generation Global Gravitational Wave Observatory: The Science Book, iii) 3G R&D: R&D for the Next Generation of Ground-based Gravitational Wave Detectors, iv) Gravitational Wave Data Analysis: Computing Challenges in the 3G Era, v) Future Ground-based Gravitational-wave Observatories: Synergies with Other Scientific Communities, and vi) An Exploration of Possible Governance Models for the Future Global Gravitational-Wave Observatory Network (this report).

==> acronyms.tex <==
\chapterimage{figures/bbh} % Chapter heading image
\chapter*{Acronyms \& abbreviations}
\addcontentsline{toc}{chapter}{\color{ocre} Acronyms and Abbreviations}
\begin{table}[h!]
\parbox{1.0\linewidth}{
\begin{tcolorbox}[standard jigsaw,colframe=ocre,colback=ocre!10!white,opacityback=0.6,coltext=black,title=\sc \large Acronyms and abbreviations used in the text]
\small
%\caption{}
\vskip-5pt
\label{tab:acronyms}
\parbox{.50\linewidth}{
	\begin{tabular}{rl}
	%\hline
	%\hline
	%{\bf Abbreviation} & {\bf Definition } \\
        % \hline 
	3G	& \emph{Third-generation}, the next generation of ground-based gravitational-wave observatories \\
	    & \emph consisting of 1 ET in Europe, 1 CE each in the US and Australia\\
	BAO	& \emph{Baryon Acoustic Oscillations} \\
	BBH	& \emph{Binary Black Hole}, a binary system of two black holes \\
	BH	& \emph{Black Hole}\\
	BNS	& \emph{Binary Neutron Star}, a binary system of two neutron stars\\
	CE	& \emph{Cosmic Explorer}, concept for a US third generation interferometer with 40 km arms \\
	CMB	& \emph{Cosmic Microwave Background} \\
	ECO	& \emph{Exotic Compact Object}, an alternative to a neutron star or a black hole \\
	EM	& \emph{Electromagnetic} \\
	ET	& \emph{Einstein Telescope}, concept for a European triangular shaped interferometer with 10 km arms\\
	GR	& \emph{General relativity} \\
	GSF	& \emph{Gravitational Self-Force} \\
	GW	& \emph{Gravitational Wave} \\
	GW150914	& Binary black hole merger event detected on 14 September 2015 \\
	GW151226	& Binary black hole merger event detected on 26 December 2015 \\
	GW170104	& Binary black hole merger event detected on 4 January 2017 \\
	GW170814	& Binary black hole merger event detected on 14 August 2017 \\
	GW170817	& Binary neutron star merger event detected on 17 August 2017 \\
	\textit{INTEGRAL} & \emph{International Gamma-Ray Astrophysics Laboratory} \\
	LIGO	& \emph{Laser Interferometer Gravitational-Wave Observatory}, 4 km arm length interferometers in \\
	     &  in the US at Hanford WA and Livingston LA\\
	LIGO-India	& LIGO interferometer being built in India \\
	\textit{LISA}	& \emph{Laser Interferometer Space Antenna} \\
	NR	& \emph{Numerical Relativity} \\
	NS	& \emph{Neutron Star}\\
	NSBH	& \emph{Neutron Star--Black Hole}, a binary system of one neutron star and one black hole \\
	PM	& \emph{Post-Minkowskian} \\
	PNS	& \emph{Proto-Neutron Star} \\
	PN	& \emph{Post-Newtonian} \\
	QCD	& \emph{Quantum Chromodynamics} \\
	SASI	& \emph{Standing Accretion Shock Instability} \\
	SM	& the \emph{Standard Model} of particle physics \\
	SN, SNe	& \emph{Supernova}, \emph{Supernovae} \\
	SNR	& \emph{Signal-to-noise ratio} \\
    Virgo & 3 km arm length interferometer located in Cascina, Italy \\
	%\hline
        %\hline
	\end{tabular}
        }
        \end{tcolorbox}
        }
        \vskip-5pt
\end{table}  
\clearpage

